Mixture Models, Robustness, and Sum of Squares Proofs

We use the Sum of Squares method to develop new efficient algorithms for learning well-separated mixtures of Gaussians and robust mean estimation, both in high dimensions, that substantially improve upon the statistical guarantees achieved by previous efficient algorithms. Firstly, we study mixtures of $k$ distributions in $d$ dimensions, where the means of every pair of distributions are separated by at least $k^{\varepsilon}$. In the special case of spherical Gaussian mixtures, we give a $(dk)^{O(1/\varepsilon^2)}$-time algorithm that learns the means assuming separation at least $k^{\varepsilon}$, for any $\varepsilon > 0$. This is the first algorithm to improve on greedy ("single-linkage") and spectral clustering, breaking a long-standing barrier for efficient algorithms at separation $k^{1/4}$. We also study robust estimation. When an unknown $(1-\varepsilon)$-fraction of $X_1,\ldots,X_n$ are chosen from a sub-Gaussian distribution with mean $\mu$ but the remaining points are chosen adversarially, we give an algorithm recovering $\mu$ to error $\varepsilon^{1-1/t}$ in time $d^{O(t^2)}$, so long as sub-Gaussian-ness up to $O(t)$ moments can be certified by a Sum of Squares proof. This is the first polynomial-time algorithm with guarantees approaching the information-theoretic limit for non-Gaussian distributions. Previous algorithms could not achieve error better than $\varepsilon^{1/2}$. Both of these results are based on a unified technique. Inspired by recent algorithms of Diakonikolas et al. in robust statistics, we devise an SDP based on the Sum of Squares method for the following setting: given $X_1,\ldots,X_n \in \mathbb{R}^d$ for large $d$ and $n = poly(d)$ with the promise that a subset of $X_1,\ldots,X_n$ were sampled from a probability distribution with bounded moments, recover some information about that distribution.

==> remaining-sos-proofs.tex <==
\section{Remaining SoS proofs}
In this section we construct the SoS proofs we deferred in the overview.

\subsection{Concentration}
The first lemma to prove is Lemma~\ref{lem:sos-centered-moments-overview}, which we will prove from two main sub-lemmas, one establishing concentration over the samples $X_1,\ldots,X_n$ and the second proving the corresponding lemma in an infinite-samples limit.

\begin{lemma}[Concentration]
\samh{TODO: need to adapt this to just use bounded moments of coefficients.}
  Let $P$ be a random degree $2d$ polynomial in $k$ indeterminates $x$.
  Let $\hat{P}(\alpha)$, the coefficients of $P$, be the scalar random variables $\hat{P}(\alpha)$ such that $P(x) = \sum_{|\alpha| \leq d} \hat{P}(\alpha) x^\alpha$ (here $\alpha$ is a multiindex of size at most $d$).
  Suppose that $D$ is a number so that $\Paren{\hat{P}(\alpha) - \E\hat{P}(\alpha)}^{1/D}$ is subgaussian with variance at most $1$, and that $\hat{P}(\alpha) = 0$ with probability $1$ if $|\alpha|$ is odd.

  Let $P_1,\ldots,P_n$ be independent samples from $P$.
Then, with probability $1 - \tau$, we have
  \begin{align*}
    \proves{2d} & \frac{1}{n} \sum_{i \leq n} P_i (x) - \E P(x) \leq   \frac{(k^d \log 1 / \tau)^{O(D)}}{n^{1/4}} (1 + \| u \|_2^2)^{d} ~\text{ and } \\
    \proves{2d} & \E P(x) - \frac{1}{n} \sum_{i \leq n} P_i (x) \leq  \frac{(k^d \log 1 / \tau)^{O(D)}}{n^{1/4}} (1 + \| u \|_2^2)^{d} \mper
  \end{align*}
\end{lemma}
\begin{proof}
By standard \jerry{TODO: actually dig up proof instead of rederiving it like I did...} moment bound arguments, there is some constant $c = c(d)$ so that for all $t > 0$ we have
\[
\Pr \Brac{\left| \frac{1}{n} \sum_{i \leq n} \hat{P}_i (\alpha) - \E \hat{P} (\alpha) \right| > t} \leq \exp \Brac{-c (nt^2)^{1 / (D + 1)}} \; ,
\]
for any $\alpha$ with $|\alpha| \leq 2d$.
Hence, by a union bound, and by setting $t = \poly \Paren{\binom{k}{2d}^D, (\log 1 / \tau)^D} \cdot \frac{1}{\sqrt{n}}$, we have
\[
\Pr \Brac{\exists |\alpha| \leq 2d: \left| \frac{1}{n} \sum_{i \leq n} \hat{P}_i (\alpha) - \E \hat{P} (\alpha) \right| > \frac{(k^d \log 1 / \tau)^{O(D)}}{\sqrt{n}}} \leq \tau \; .
\]
Condition on the event that
\begin{equation}
\label{eq:monomial-bound}
\left| \frac{1}{n} \sum_{i \leq n} \hat{P}_i (\alpha) - \E \hat{P} (\alpha) \right| < \frac{(k^d \log 1 / \tau)^{O(D)}}{\sqrt{n}}\; , ~\forall |\alpha| \leq 2d
\end{equation}
occurs for the rest of the proof.
For all $s \geq 0$, let $Q_s(x)$ be the degree $s$ component of $\frac{1}{n} P_i (x) - \E P(x)$.
Conditioned on \eqref{eq:monomial-bound} holding, by Fact~\ref{fact:poly-moment-bound}, we know that with
\[
\proves{O(d)} Q_s (x) \leq \Paren{ \frac{(k^d \log 1 / \tau)^{O(D)}}{\sqrt{n}}}^{1/2} \| u \|_2^{2 \lceil s \rceil} \; ~~\mbox{and}~~ \proves{O(d)} -Q_s (x) \leq \Paren{ \frac{(k^d \log 1 / \tau)^{O(D)}}{\sqrt{n}}}^{1/2} \| u \|_2^{2 \lceil s \rceil} \; .
\]
Since the overall degree of the polynomial is even, the first bound implies 
\[
\proves{2d} \frac{1}{n} \sum_{i \leq n} P_i (x) - \E P(x) \leq   \Paren{ \frac{(k^d \log 1 / \tau)^{O(D)}}{\sqrt{n}}}^{1/2} \sum_{s = 1}^d \| u \|_2^{2s} \leq  \frac{(k^d \log 1 / \tau)^{O(D)}}{n^{1/4}} (1 + \| u \|_2^2)^{d} \; ,
\]
and similarly the second bound gives
\[
\proves{2d} \E P(x) - \frac{1}{n} \sum_{i \leq n} P_i (x) \leq  \frac{(k^d \log 1 / \tau)^{O(D)}}{n^{1/4}} (1 + \| u \|_2^2)^{d} \; ,
\]
which completes the proof.
\end{proof}


\begin{lemma}[Infinite-samples version of Lemma~\ref{lem:sos-centered-moments-overview}]
  Let $u = (u_1,\ldots,u_k)$ be a $k$-length vector of indeterminates.
  Let $t \in \N$ be a power of $2$.
  Let $\cD$ be a centered, $10t$-explicitly bounded distribution.
  Let $X,Y \sim \cD$.
  Then
  \[
    \proves{O(t)} \E_Y\Brac{\Paren{\iprod{u, Y + u} - \E_X\Brac{ \iprod{u,X+u}}}^t} \leq (t)^{O(t)} \cdot (1 + \|u\|_2^2)^{t/2}\mper
  \]
\end{lemma}
\begin{proof}
  We start by applying Theorem~\ref{thm:sos-2-to-q} to the function $f(Y) = \iprod{u, Y + u}^t - \E_X\Brac{ \iprod{u,X+u}^t}$, itself a polynomial in indeterminates $u$, to obtain
  \begin{equation}
  \label{eq:infinite-samples-1}
  \proves{O(tq)} \E_Y\Brac{\Paren{\iprod{u, Y + u}^t - \E_X\Brac{ \iprod{u,X+u}^t}}^q} \leq (q-1)^{qt/2} \Paren{\E_Y \Brac{\Paren{\iprod{u, Y + u}^t - \E_X\Brac{ \iprod{u,X+u}^t}}^2}}^{q/2}\mper
  \end{equation}
  We expand the $t$-th power to get
  \[
    \iprod{u, Y + u}^t - \E_X\Brac{ \iprod{u,X+u}^t} = \sum_{s \leq t} \binom{s}{t} \cdot \|u\|_2^{2s} (\iprod{u,Y}^{t-s} - \E_X \iprod{u,X}^{t-s})
  \]
  and use Cauchy-Schwarz:
  \[
  \proves{O(t)} \Paren{\sum_{s \leq t} \binom{s}{t} \cdot \|u\|_2^{2s} (\iprod{u,Y}^{t-s} - \E_X \iprod{u,X}^{t-s})}^2 \leq t^{O(t)} \cdot \sum_{s \leq t} \|u\|_2^{4s} (\iprod{u,Y}^{t-s} - \E_X \iprod{u,X}^{t-s})^2\mper
  \]
  The $s = t$ term is zero.
  Now we bound the rest.
  First we use Fact~\ref{fact:sos-gaussian-moment}, which says that 
  \[
    \proves{2a} \E_Y \iprod{Y,u}^{2a} \leq (2a)! \cdot \|u\|_2^{2a}\mper
  \]
  Expecting over $Y$, this allows us to bound the $s$-th term by $4 t! \cdot \|u\|_2^{2s + 2t}$, so we obtain
  \[
  \proves{O(t)} \E_Y \Brac{\Paren{\iprod{u, Y + u}^t - \E_X\Brac{ \iprod{u,X+u}^t}}^2} \leq 4 t^{O(t)} (1 + \|u\|_2^2)^{2t-1} 
  \]
  where we have used the easy-to-check fact $\proves{O(t)} \sum_{s \leq t-1} \|u\|_2^{2s} \leq (1 + \|u\|^2)^{t-1}$.
  Combining this with \eqref{eq:infinite-samples-1} finishes the proof.
\end{proof}

\subsection{Proof of Lemma~\ref{lem:overview-pairs}}
\samh{need to adapt to remove the $q$ stuff}
We are now ready to put together the pieces we have developed in the preceding section and the proof overview (Section~\ref{sec:overview-ident-mixtures}) to prove the main SoS identifiability statement, Lemma~\ref{lem:overview-pairs}.
\newcommand{\cB}{\mathcal{B}}
We will prove the lemma as a corollary of the following proposition, which captures in SoS some simple reasoning about magnitudes of error terms in the lemmas we are putting together.
\begin{proposition}
\label{prop:ugly-sos}
  Let $x,y,z,w$ be indeterminates and $t,q$ be powers of $2$, with $t,q > 1$.
  Let $\calB$ be the following set of inequalities.
  \begin{align}
    & x^{q/2} y^{tq}  \leq A y^{tq/2} + B x^{q/2-1}(1+y)^{(t-1)q} \label{eq:B1}\\
    & w^{q/2} z^{tq}  \leq A z^{tq/2} + B w^{q/2-1}(1+z)^{(t-1)q} \label{eq:B2}\\
    & (1+y)^{tq} + (1+z)^{tq}  \geq C \label{eq:B3} \\
    & x \leq D \label{eq:B4} \\
    & w \leq D \label{eq:B5}\\
    & (1 + y) \leq G \label{eq:B6}\\
    & (1 + z) \leq G \label{eq:B7}
  \end{align}
  where $A,B,C,D,G$ are scalars.
  Then
  \[
    \calB \proves{O(tq)} x^q y^q \leq \frac{2^{O(qt)}}{C} \cdot \Brac{D^q + B^q + D^{q-1}B} \Paren{D^q + A^2 + BD^{q-1} C^{1/2} + \frac{2^{O(tq^2)} B^q G^{tq}}{C^{q/(2t-2)}}}
  \]
\end{proposition}
\begin{remark}[Understanding Proposition~\ref{prop:ugly-sos}]
To understand the proposition in the broader context of this paper, the reader may think of the following correspondences.
\begin{align*}
  x &  \iprod{a_i,w}\\
  w & = \iprod{a_j,w}\\
  y & = \|v_i\|^2\\
  z & = \|v_j\|^2\\
  A & \approx n^{q/2}\\
  B & \approx n\\
  C & \approx \Delta^{2tq}\\
  D & \approx n\\
  G & \approx \poly(k)
\end{align*}
where $\Delta$ is the minimum distance between Gaussian centers.
With these parameters, the conclusion of the proposition becomes (roughly)
\[
  \calB \proves{O(tq)} \iprod{a_i,w}^q \iprod{a_j,w}^q \leq \frac{2^{O(tq)}}{\Delta^{2tq}} \cdot n^q \cdot \Paren{n^q + \Delta^{tq} n^q + \frac{2^{O(tq^2)} n^q k^{O(tq)}}{\Delta^{q^2/2}}}\mper
\]
If $\delta = k^\e$, then picking $q \gg t/\e$, the last term is at most $n^q$, and the whole thing is at most $2^{O(tq)} n^{2q} / \Delta^{tq}$.
Then choosing $t \gg 1/\e$, the bound becomes $n^{2q} / k^{100q}$ as desired.
\end{remark}

\samh{put the ugly munge-y lemmas here}

\subsection{Graveyard}
\subsection{Proof of Lemma~\ref{lem:ugly-sos-2}}
In this section we prove Lemma~\ref{lem:ugly-sos-2} by assembling some standard SoS tools.

\begin{fact}
  \label{fact:sos-univ-1}
  For every $c > 0$ and even $q \in \N$, the polynomial $p(X) = X^q - c X^{q-1} + c^q$ is a sum of squares.
\end{fact}
\begin{proof}
  Since $p$ is univariate it is enough to show it is everywhere nonnegative.
  If $|X| \geq c$ then $X^q \geq c X^{q-1}$, while if $|X| \leq c$ then $c^q \geq c X^{q-1}$.
\end{proof}

\begin{fact}
\label{fact:interval-bound}
For any positive scalars $\alpha, \beta$, and for any $t \geq 1$, we have $\proves{O(t)} (\alpha - \beta x^2) x^{2 (t - 1)} \leq \alpha (\alpha / \beta)^{t - 1}$.
\end{fact}
\begin{proof}
Since this is a univariate statement about degree $O(t)$ polynomials, it suffices to show that the inequality $(\alpha - \beta x^2) x^{2(t - 1)} \leq \alpha (\alpha / \beta)^{t - 1}$ holds for all $x \in \R$.
If $x \not\in [0, \sqrt{\alpha / \beta}]$ then the LHS is negative, and so the inequality holds.
On the other hand, if $x \in [0, \sqrt{\alpha / \beta}]$, then we have $( \alpha - \beta x^2) \leq \alpha$ and $x^{2(t - 1)} \leq (\alpha / \beta)^{(t - 1)}$, and so the inequality holds.
This concludes the proof.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:ugly-sos-2}]
  Starting with evenness of $q$ and Fact~\ref{fact:sos-univ-1}, we get
  \[
    \proves{O(t)} x_0^t x_1^t \leq (2 x_0^t - c x_0^{t-1} + c^t)(2 x_1^t - c x_1^{t-1} + c^t)
  \]
  for $c \in \R$ to be chosen later.
  Since $2 x^t - c x^{t-1} + c^t$ is a sum of squares, we can use the lower bound on $y_0^t + y_1^t$ to obtain that
  \[
   \calB \proves{O(t)} x_0^t x_1^t \leq \frac{y_0^{2t} + y_1^{2t}}{B} \cdot (2 x_0^t - c x_0^{t-1} + c^t)(2 x_1^t - c x_1^{t-1} + c^t)\mper
  \]

  By symmetry, to prove the lemma it will be enough to bound $y_0^{2t} (2 x_0^t - c x_0^{t-1} + c^t)(2 w_1^t - c x_1^{t-1} + c^t)$.
  Let $E := 2 C^t + c C^{t-1} + c^t$.
  Then by univariateness and the bound $x_i \leq C$ in $\calB$,
  \[
    \calB \proves{O(t)} (2 x_1^t - c x_1^{t-1} + c^t) \leq E
  \]
  and hence
  \begin{align}
    \label{eq:sos-bs-1}
    \calB \proves{O(t)} y_0^{2t} (2 x_0^t - c x_0^{t-1} + c^t)(2 w_1^t - c x_1^{t-1} + c^t) \leq E \cdot y_0^{2t} (2 x_0^t - c x_0^{t-1} + c^t)\mper
  \end{align}
  Dropping the subscript now, we work on the term
  \samh{revising here}
  Now we work on the term $(1+y)^{tq} x^q$.
  We know
  \[
  \calB \proves{O(tq)} (1+y)^{tq} x^q \leq 2^{O(tq)} \cdot (1 + y^{tq}) \cdot x^q \leq 2^{O(tq)}\cdot  D^q + 2^{O(tq)}\cdot y^{tq} x^q\mper
  \]
  We need to get set up to cancel some terms coming out of \eqref{eq:B1}.
  We add the square $2^F (A - x^{q/2}y^{tq/2})^2$ (we will choose the scalar $F$ later) to obtain
  \[
    \calB \proves{O(tq)} (1+y)^{tq} x^q \leq 2^{O(tq)}\cdot  D^q + 2^{O(tq)}\cdot y^{tq} x^q + 2^F A^2 + 2^{F} x^q y^{tq} - 2 \cdot A \cdot 2^{F} \cdot x^{q/2} y^{tq/2}
  \]
  and grouping terms,
  \[
  \calB \proves{O(tq)} (1+y)^{tq} x^q \leq 2^{O(tq)}\cdot D^q + 2^{O(tq) + F}\cdot y^{tq} x^q + 2^F A^2 - 2 \cdot A \cdot 2^{F} \cdot x^{q/2} y^{tq/2}\mper
  \]
  Now we apply \eqref{eq:B1} to get
  \[
    \calB \proves{O(tq)} (1+y)^{tq} x^q \leq 2^{O(tq)}\cdot D^q + 2^{O(tq) + F}\cdot x^{q/2} \cdot ( A y^{tq/2} + B x^{q/2-1}(1+y)^{(t-1)q}) + 2^F A^2 - 2 \cdot A \cdot 2^{F} \cdot x^{q/2} y^{tq/2}\mper
  \]
  Now choosing $F$ as some constant multiple of $qt$ in order to cancel terms, we get
  \begin{align}
  \label{eq:sos-bs-2}
  \calB \proves{O(tq)} (1+y)^{tq} x^q \leq 2^{O(tq)}\cdot \Brac{D^q + B x^{q-1}(1+y)^{(t-1)q} +  A^2 }\mper
  \end{align}

  It's time to return to \eqref{eq:sos-bs-1}.
  Plugging in \eqref{eq:sos-bs-2} into the right-most entry in \eqref{eq:sos-bs-1}, we get
  \begin{align*}
    \calB \proves{O(tq)} & E \cdot (1 + y)^{tq} \cdot (2 x^q - cx^{q-1} +c^q)\\
    & \leq E \cdot \Brac{ 2^{O(tq)} \cdot \Brac{D^q + B x^{q-1}(1+y)^{(t-1)q} +  A^2 } -  (1+y)^{tq} \cdot c x^{q-1} + (1+y)^{tq} c^q }\\
    & = E \cdot 2^{O(tq)} \cdot (D^q + A^2) + E \cdot \underbrace{(1+y)^{tq} c^q}_{=: p(y)} + E \cdot \underbrace{x^{q-1} (1+y)^{(t-1)q} ( 2^{O(tq)} \cdot B - c(1+y)^{q})}_{ =:r(x,y)}\mper
  \end{align*}
  We claim there is a choice of $c$ so that 
  \[
    \calB \proves{O(tq)} r(x,y) \leq 2^{O(tq)} B D^{q-1} C^{1/2} \text{ and } \calB \proves{O(tq)} p(y) \leq \frac{2^{O(tq^2)} G^{tq} B^q} {C^{\tfrac{q}{2(t-1)}}}
  \]
  Choose $c = 2^{O(tq)} B/C^{\tfrac 1 {2(t-1)}}$.
  Then these follow from Fact~\ref{fact:interval-bound} and the inequalities in $\calB$, in particular \eqref{eq:B4} and \eqref{eq:B6}.
  Following the inequalities back through completes the proof.
\end{proof}



